Distributed Bounded Model Checking

Program verification is a resource-hungry task. This paper looks at the problem of parallelizing SMT-based automated program verification, specifically bounded model-checking, so that it can be distributed and executed on a cluster of machines. We present an algorithm that dynamically unfolds the call graph of the program and frequently splits it to create sub-tasks that can be solved in parallel. The algorithm is adaptive, controlling the splitting rate according to available resources, and also leverages information from the SMT solver to split where most complexity lies in the search. We implemented our algorithm by modifying CORRAL, the verifier used by Microsoft's Static Driver Verifier (SDV), and evaluate it on a series of hard SDV benchmarks.

==> sections/client.tex <==
\subsection{Client-Side Verification Algorithm}
\label{Se:Client}

\begin{algorithm}[t]
\DontPrintSemicolon
\KwIn{A Program $P$}
\KwIn{An SMT solver $\solver$}
\While{true \label{Ln:ClientInfiniteLoop}}  {
    $\solver$.reset() \; \label{Ln:SolverReset}
    $\rho \gets \callServer$(\texttt{GET\_PARTITION}) \; \label{Ln:GetPartition}
    outcome $\gets$ \textsc{Verify}($P$, $\rho$, $\solver$) \; \label{Ln:CallVerify}
    $\callServer$(\texttt{OUTCOME}, outcome) \; \label{Ln:ReturnOutcome}
    }
\caption{Client-side verification algorithm}
\label{Alg:Client}
\end{algorithm}

The client-side implementation of $\toolname$ is shown in \algoref{Client}.
The routine $\callServer$ is used for sending a message to the server. The first argument to $\callServer$
is the message \textit{type}, and the rest of the arguments form the message \textit{payload}. When a call to this routine does not expect a return value,
we assume that the message is sent asynchronously.
When we expect a return value, we assume a send-receive roundtrip that also fetches a response
from the server (i.e., it blocks until the server's response arrives).
Further, we assume that each client has a globally unique identifier and each message sent by the
client implicitly contains this ID so that the server can identify the sender.

The client runs an infinite loop (\lineref{ClientInfiniteLoop}). (In practice, the server sends a special message to
kill all clients when the program verification finishes; we do not show this exchange for
simplicity.)
Inside the loop, the client resets its solver (which discards all previously asserted constraints)
to get ready for the next verification sub-task. It gets a partition from the server (\lineref{GetPartition})
and starts solving it (\lineref{CallVerify}). The bulk of verification happens in the
\textsc{Verify} procedure. As part of solving a partition, the client can
create new partitions by splitting search and send them to the server. The client goes \textit{idle}
when it finishes a partition with a \textsc{Safe} or \textsc{UnSafe} verdict, in which case it sends
the outcome to the server (\lineref{ReturnOutcome}) and repeats its infinite loop.

Splitting works by picking an
arbitrary dynamic callsite $c$ (that has already been inlined) and deciding to either force the
program execution to go through the callsite or definitely not go through it. This split results in
two mutually-disjoint (but together exhaustive) search spaces. A splitting \textit{decision} is
either $\texttt{BLOCK}(c)$ or $\texttt{MUSTREACH}(c)$ depending on whether we are blocking the
callsite $c$ or declaring that $c$ must be taken. A \textit{partition} is a pair
$(T, D)$ where $T$ is the call tree (i.e., set of inlined callsites) and $D$ is a set of decisions.
As a notation shorthand, for a partition $\rho = (T, D)$ and callsite $c$, let $\rho + c$
be the partition $(T \cup \{ c \}, D)$. Similarly, for a decision $d$, let $\rho
+ d$ be the partition $(T, D \cup \{ d \})$. Further, let $\calltree((T,D)) = T$
and $\decisions((T, D)) = D$.

The \textsc{Verify} routine is outlined in \algoref{Verify}. The local
variable $dstack$ will be used to maintain a stack of decisions that the routine
will make. $C$ will maintain the set of open callsites, similar to SI,
and $uc$ will store the unsat core obtain from the last solver call.

The routine starts by
preparing the input partition (\linesref{SetupBegin}{SetupEnd}). This requires
inlining the input call tree. The \textsc{Inline} routine is used to inline
open calls. It follows from stratified inlining (essentially \linesref{InlineBegin}{InlineEnd} of
\algoref{SIStep}). Next, we assert the input decisions. Blocking
a callsite $c$ is easy: we assert $\neg \cvar(c)$. Asserting that a
callsite must be taken requires more care; we detail the $\mr$ constraint later
in this section.

The loop that follows (\lineref{VerifyLoop}) works until it can reach a
\textsc{Safe} or \textsc{UnSafe} verdict, however, it can split the search
in-between, thus, its returned outcome holds for the final partition it was
solving, not necessarily
the input partition. (The rest of the work is farmed back to the server.) In
\lineref{whensplit}, we make a non-deterministic choice of whether to split or
not. (The exact heuristic is explained in \sectref{SplitRate}.)
If we decide to split, we pick a callsite $c$ to split on (\lineref{findsplit}).
The only constraint is that $c$ must have already been inlined, i.e., $c \in
\calltree(\rho)$. The choice of splitting callsite is informed by the unsat core computed in a
previous iteration of the loop (see \sectref{SplittingHeuristic}).
\linesref{SplitBegin}{SplitEnd} perform the split on $c$ such that the current client continues to
work on the partition where $c$ is blocked. This requires setting a backtracking point
on the solver (via \texttt{Push}). The splitting decision is recorded in variables $dstack$ and $\rho$ and the must-reach
partition is sent over the server. Setting of the backtracking point in the solver is important:
if the client finishes search on the block partition with a \textsc{Safe} verdict, it will attempt
to \textit{steal} the must-reach partition from the server (\lineref{PartitionSteal}).

\input{verify.tex}

Once the splitting is done, the \textsc{Verify} routines calls \textsc{SIStep}
(\lineref{VerifyCallSIStep}) to proceed with its search in the current partition ($\rho$).
If a counterexample is found, we can immediately return an \textsc{UnSafe} verdict back to the
server to conclude the search across all clients. If \textsc{SIStep} returned \textsc{NoDecision}, it
must have inlined more procedures, so we update local variables and iterate. Finally, if
\textsc{SIStep} returned \textsc{Safe}, then the search on the current partition has finished and
the client must pick another partition to solve. This is done by returning the \textsc{Safe} verdict
(\lineref{VerifySafe}). The check on \lineref{PartitionSteal} is an optimization. The client checks
with the server if the last partition that it sent is still with the server (i.e., it has not been
farmed out to another client). If so (server returns \texttt{YES}), then the client
steals the partition and starts working on it immediately. In order to do so, it just backtracks the
solver state via \texttt{Pop}, asserts the $\mr$ constraint,and continues. Backtracking the solver is much cheaper than having a
different client go through the entire setup for the partition (\linesref{SetupBegin}{SetupEnd}).
The flipped decision is recorded in $dstack$ and $\rho$ variables. Note that the loop on
\lineref{PopLoop} is needed: only \texttt{BLOCK} decisions are flipped, the \texttt{MUSTREACH}
decisions are always just popped off.

\subsection{When to split?}
\label{Se:SplitRate}

Splitting is essential to obtain parallelism, however, splitting too much can
introduce unnecessary overheads. Ideally, we should split just enough to keep all
clients busy all the time. We control the rate of splitting in
proportion to the number of idle clients, and inversely
proportional to the number of partitions already available at the server. In
other words, a client will split at a faster rate if there are a large number of idle
clients and the server has comparatively lesser number of partitions available.

Each client maintains a \textit{split time interval} $\delta$ (in seconds).
It splits the search if $\delta$ seconds have elapsed since the last split.
The value of $\delta$ is initially $\delta_c$ (a fixed constant) but it can be updated
by the server. The server sends this value back as a reply to the
$\texttt{SEND\_PARTITION}$ message.
The server computes $\delta_i$ for a client $i$ as follows:

\begin{equation}\label{sprate}
\delta_i =
    \begin{cases}
      \frac{Q[i].count}{wt.count}\times \delta_c & \mbox{if } wt.count \neq 0 \\
      K \times \delta_c, & \mbox{otherwise}.
    \end{cases}
\end{equation}

In the first case, a client's splitting is slowed down in proportion to its queue size
(divided by the number of idle clients).
The second case applies when there are no idle clients. Increasing $\delta$ by a
factor of $K$ reduces the rate of splitting drastically. We use the values
$\delta_c=0.5s$ and $K=20$ in our experiments.

==> sections/conclusion.tex <==
\section{Conclusions}
\label{Se:Conclusions}

We propose a distributed architecture for program verification based on the stratified inlining algorithm
using a proof-guided dynamic partitioning algorithm. The success of our partitioning-based approach and the high variance on
our priliminary experiments with randomization (indicating a heavy-tailed distribution) points to a
possibilities on interesting hybid schemes: in the future, we are interested in exploring hybrid
partitioning-portfolio approch with randomized task-splitting heuristics.


==> sections/heuristic.tex <==
\subsection{Proof-Guided Splitting}
\label{Se:SplittingHeuristic}

This section describes the implementation of the \textbf{choose} operation used in
\lineref{findsplit} of \algoref{Verify}. As mentioned in \sectref{Introduction}, our goal is to find
proof-disjoint splits.

Given an unsatisfiable formula $\Phi$, expressed as a conjunction set of clauses $\{\phi_i\}$,
a \textit{minimal unsatisfiable core} is a subset of clauses $\Psi \subseteq \Phi$ who conjunction is
still unsatisfiable, and every proper subset of $\Psi$ is satisfiable. Whenever an under-approximate
check is unsatisfiable, we extract the minimal unsat core to capture its proof of unsatisfiability.
Each conjunct in our checks corresponds to either an inlined callsite or an open callsite that we
are blocking. We, thus, represent the unsat core as a set of callsites. We call these callsites as
\textit{proof-relevant}; our goal is to break these unsat proofs by splitting.

Let $T$ be the set of inlined callsites at some point and let $uc$ be the unsat core obtained from
an unsatisfiable under-approximate query. Let $\texttt{subtree}(T, c)$ be the subset of $T$ that
contains all callsites $c' \in T$ such that $c$ is a prefix of $c'$. In that case, we choose the
splitting callsite as follows:
$\underset{c \in uc}{\texttt{argmax}} \{ | \texttt{subtree}(T, c)\cap uc| \}$



%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}[t]
  %\centering
    \vspace{-20pt}
  \includegraphics[width=\linewidth]{figures/inliningTree3}
    \vspace{-25pt}
    \caption{\label{fig:splitting}Proof-guided splitting}\label{split}
\end{figure}
%\end{wrapfigure}


\Omit{
We explain this choice through an example. Consider the inlining tree shown in
Figure~\ref{fig:splitting}, where the open callsites appear as dotted circles
and inlined ones are shown as solid circles. Further, assume that the shaded nodes are the callsites
that appear in the unsat core $uc$. We can split on any inlined callsite, and clearly there is no
point splitting on \texttt{main}. The callsite \texttt{baz} does not appear on the unsat core. If we
split on it, then the same unsat core would still hold for both sides of the split. Choosing a
%callsite on the unsat core breaks that unsat-proof. Between \texttt{foo} and \texttt{bar}, we pick
the one that has more proof-relevant descendants, i.e., \texttt{bar}. Blocking on \texttt{bar}
makes the descendants of \texttt{foo} relevant, whereas a must-reach on \texttt{bar} makes its own
descendants relevant, creating a more balanced split.
}

\Omit{
\begin{enumerate}
    \item[\texttt{baz}] This callsite does not appear on the unsat core. If we split on it, the same
	    unsat core would still hold for both sides of the split.
    \item[\texttt{foo}] Being a proof-relevant call-site, by the above property of unsatisfiability cores, blocking on this call-site (equivalent to removing the VC of \texttt{foo} from the program encoding) will render the current proof of satisfiability useless, forcing the solver to search for a different proof. The current proof, however, continues to hold in the mustreach encoding (as it retains all terms in the original VC) and, thus, can explore its outcomes on refinements of the program;
    \item[\texttt{bar}] For the same reason as above, \texttt{bar} is also a good candidate for splitting. However, choosing a split-candidate that is heavy with proof-relevant descendents in its subtree tends to create more \textit{balanced} partitions: its descendents in one partition, while all the rest of its siblings and their descendents in the other\footnote{we also experimented with heuristics that explicitly select candidates that divide the proof-relevant call-sites equally; we achieved similar performance with both and preferred the former for its simplicity.}
\end{enumerate}


The above property ensures that removal of any clause $\phi_i\in \Psi$ from $\Phi$ either renders $\Phi \setminus \phi_i$ satisfiable, or a \textit{different proof} is found (with an unsatisfiable core $\Phi'$ such that $\Phi' \not\subset \Phi$). As discussed in the introduction, selecting any arbitrary call-site as the split candidate would ensure \textit{path disjointness}, but not necessarily \textit{proof disjointness}; we use the above property of minimal unsatisfiable cores in a search for proof disjointness.

Figure~\ref{fig:splitting} shows an inlining tree, where the open call-sites appears as dotted circles while the inlined call-sites are shown as solid circles. Assuming that the underapproximate query (i.e. where all open call-sites are \textit{blocked}) is unsatisfiable, we may extract a \textit{minimal unsatisfiable core} to capture the proof of unsatisfiability. Let us assume that the shaded nodes correspond to the call-sites $c_i\in C$ such that the logical encoding of basic-blocks containing $c_i\in C$ appear in the minimal unsatisfiability core; we refer to such call-sites that appear in the minimal unsatisfiability core as \textit{proof relevant} call-sites.


At this stage, we have three choices for the split candidate:
\begin{enumerate}
    \item[\texttt{baz}] As this call-site is not proof-relevant, the current proof of unsatisfiability will still hold on both its block and mustreach lemmas;
    \item[\texttt{foo}] Being a proof-relevant call-site, by the above property of unsatisfiability cores, blocking on this call-site (equivalent to removing the VC of \texttt{foo} from the program encoding) will render the current proof of satisfiability useless, forcing the solver to search for a different proof. The current proof, however, continues to hold in the mustreach encoding (as it retains all terms in the original VC) and, thus, can explore its outcomes on refinements of the program;
    \item[\texttt{bar}] For the same reason as above, \texttt{bar} is also a good candidate for splitting. However, choosing a split-candidate that is heavy with proof-relevant descendents in its subtree tends to create more \textit{balanced} partitions: its descendents in one partition, while all the rest of its siblings and their descendents in the other\footnote{we also experimented with heuristics that explicitly select candidates that divide the proof-relevant call-sites equally; we achieved similar performance with both and preferred the former for its simplicity.}
\end{enumerate}

Now to state our heuristic formally, let $T$ be the inlining tree, and \texttt{subtree}(T, c) returns the subtree rooted at c. Given a proof of unsatisfiability
that returns a set of \textit{proof relevant} calls-sites (\textit{R}):
%$$pr(uc) = \{c : c\in b \land b \in uc\}$$

\begin{align}
\underset{c \in R}{\texttt{argmax}} [\texttt{size}(\texttt{subtree}(T, c)\cap R)]
\end{align}
\vspace{2pt}

That is, we split on the call sites that contains the largest number of
proof-relevant call-sites in its subtree. We show the partitions that are likely to be obtained by splitting by our heuristic in different colors.

We note that this choice is a heuristic. It can fail, for instance, if there are control-dependencies
between callsites. For instance, if the call to \texttt{bar} dominates the call to \texttt{foo}
in the control-flow graph of \texttt{main}, blocking on \texttt{bar} also blocks
control-flow through \texttt{foo}, thereby rendering one side of the split on \texttt{bar} to be
trivial. Furthermore, in practice, we do not insist on obtaining a \textit{minimal} unsat core (solvers like Z3 provide best-effort unsat core minimization via the \texttt{core.minimize} option).

\Omit{
    However, the above heuristic may fail to provide good split candidates due to two simplifying assumptions in our analysis:

\begin{enumerate}
    \item We use a \textit{flow-insensitive} model of the program, assuming no knowledge of the control-flow. For example, if \texttt{bar} dominates \textit{foo} in the control-flow graph of \texttt{main}, blocking on \texttt{bar} also blocks control-flow through \texttt{foo}, thereby rendering one partition containing the subtrees of both \texttt{foo} and \texttt{bar} on one partition, and a (possibly trivial) subtree of \texttt{baz} on the other;
    \item We assume a procedure to compute a minimal unsatisfiability core in the preceeding discussion; however, unsatisfiable cores of modern SMT solvers may not be minimal\footnote{The newer versions of Z3 attempt best-effort unsat core minimization with the \texttt{core.minimize} option}.
\end{enumerate}
}
}


%We now explain the motivation behind this splitting heuristic.  Consider the example of an inlining tree shown in Figure \ref{split}. Assume that the callsites $A$, $C$ and all their descendants modify some variable $x$ in $Main$ and the termination of $Main$ is dependant on an assertion on $x$. As per our definition of the inlining tree, we know that the leaf nodes are non-inlined, i.e., they are open and are a candidate to be inlined next should they appear on an error trace. Let us assume that we fire an underapproximation query at this stage by blocking \{A1, A2, B1, C11, C12, C21, C31, C32\} which is \texttt{UNSAT} and the minimal unsat core returns the labels of \{A, A1, A2, C, C1, C2, C3, C11, C12, C21, C31, C32\}. Intuitively, we can understand that the unsat core signifies that had we opened even one of the open callsites on the unsat core, the unsat query may have become \texttt{SAT}. This means, when we fire an overapproximation query, if the query \texttt{SAT}, the error trace will contain at least one or more of the callsites from the unsat core. Since, our objective is to split a program into two proof-disjoint partitions such that both partitions inline different set of callsites, it makes sense to split on some callsite $\sigma$ from the unsat core. If we do this, we can expect the mustreach partition will likely inline descendants of $\sigma$ and the block partition will inline some callsites other than $\sigma$.

%Hence, when we split, we choose our split site from the set of the callsites on the unsat core. However, there can be many such callsites. How do we pick the best possible callsite such that the inlinings on both partitions are highly likely to be distinct? To answer this, we again look at the inlining tree in Figure \ref{split}. As we can see that, disregarding the root $Main$, more descendants of $C$ are being inlined in order to verify the program. This signifies that most of the error traces we have found so far must have contained $C$ or descendants of $C$. Since, the subtree of $C$ contains the most number of unsat core nodes, if we block $C$, it is likely that we will explore some other part of the program, i.e., inline some callsites other than the descendants of $C$, in order to verify it. We design our splitting heuristic based on this intution. Whenever, we decide split, we select an inlined callsite whose subtree contains the most number of unsat core nodes.



==> sections/implementation.tex <==
%\subsection{Design of the distributed system}
%\begin{figure}
%  \centering
%  \includegraphics[width=1\linewidth, height=20 cm]{figures/messageDiagram}
%  \caption{Message diagram depicting communication between server, listener and client}\label{message}
%\end{figure}

%\begin{figure}
%  \centering
%  \includegraphics[width=1\linewidth]{figures/architecture}
%  \caption{\toolname{} architecture}\label{message}
%\end{figure}
%
%We use the following APIs to describe our algorithm:
%
%\begin{itemize}
%    \item $\callServer$(Msg, ...)
%    \item Setup(solver, partition)
%    \item ReceiveMessage()
%\end{itemize}
%
%Following are the APIs for the solver:

%\begin{itemize}
%    \item CreateSolver: Creates a new instance of SMT solver
%    \item Push: Starts a new scope
%    \item Pop: Removes any assertions after the matching Push
%    \item Assert: Asserts a set of logical expressions onto the prover stack
%    \item Model: Gets the satisfiable assignment for a SAT query
%    \item UnsatCore: Extracts the Unsat Core for an UNSAT query
%    \item Check: Checks whether a given query is satisfiable or not
%\end{itemize}

%\begin{table}
%  \centering
%  \begin{tabular}{l|r}
%    \hline
%    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%    Message From Client & Reply From Server \\
%    \hline
%    \texttt{ID} & Integer ID of Client \\
%    \texttt{SEND\_PARTITION} & Steals A Partition From Another Client\\
%    \texttt{GET\_PARTITION} & Updated Splitting Speed \\
%    \texttt{POP} & \texttt{YES} or \texttt{NO} \\
%    \texttt{OUTCOME} & \texttt{CONTINUE} or noReply \\
%    \hline
%  \end{tabular}
%  \caption{Communication between server and client}\label{comm}
%\end{table}

\subsection{Server Implementation}
\label{Se:Server}

The server plays the role of an administrator in \toolname. Whenever a
client splits, it immediately starts working on the \texttt{BLOCK} partition and
sends the \texttt{MUSTREACH} partition to the server while also saving the
partition in its own local solver stack. The server stores the \texttt{MUSTREACH}
partitions and distributes them to other idle clients. The server is responsible
for balancing load across the clients.
%In this way, we can balance
%the load of work across different clients. We discuss the load-balancing in more
%detail later.

\begin{algorithm}[t]
\KwIn{A message $m$ sent by a client \textit{id}}
\KwIn{Array of double-ended queues $Q$, indexed by client \textit{id}}
\KwIn{Queue $wt$ of waiting clients}
    \If {m == $\langle\texttt{SEND\_PARTITION}, \rho\rangle$} {\label{Ln:l1}
            $Q[id]$.PushLeft($\rho$)\;\label{Ln:l2}
        }
    \ElseIf { m == $\langle\texttt{POP} \rangle$} {\label{Ln:l4}
            \If {Q[\textit{id}] $\neq \emptyset$} {\label{Ln:l5}
                Q[\textit{id}].PopLeft()\;\label{Ln:l6}
                Reply(\textit{id}, \texttt{YES})\;\label{Ln:l7}
            }
            \Else {
                Reply(\textit{id}, \texttt{NO})\;\label{Ln:l8}
            }
        }
    \ElseIf {m == $\langle \texttt{GET\_PARTITION} \rangle$} {\label{Ln:l9}
         $wt$.Enqueue(\textit{id})\;\label{Ln:l10}
        }
    \While {$wt \neq \emptyset \land \exists j. Q[j].count > 0$} {\label{Ln:l11}
                $i \gets \underset{j}{argmax}$ Q[$j$].count\;\label{Ln:l12}
                $r \gets$ $wt$.Dequeue()\;\label{Ln:l13}
                Reply($r$, Q[$i$].PopRight())\;\label{Ln:l14}
            }

\caption{Server-side implementation}
\label{Alg:Server}
\end{algorithm}


%\begin{figure}[t]
%  \centering
%  \includegraphics[width=1\textwidth]{figures/deq}
%  \caption{Maintaining the double-ended queues}
%\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.6]{figures/deq2}
  \caption{\label{Fi:deqFig}Maintaining the double-ended queues}
\end{figure}

The server waits for messages from clients and responds to them. The
implementation is shown in \algoref{Server}. The server has two key important
data structures. It maintains an array $Q$ of double-ended queues (that allow
dequeue operations from both ends). The array is indexed by client \textit{id}.
The operations on $Q$ are illustrated in \figref{deqFig}.

\textcolor[rgb]{1.00,0.00,0.00}{Note that, we have opted to implement $Q$ as an array of double-ended queues rather than a centralized single queue as used in classical work-stealing. This ensures that a client, on finishing a block partition, can immediately pick up the corresponding must-reach (last sent) without any extra overhead. On the other hand, while stealing work, a client picks up the earliest partition so that the re-initialization overhead is reduced. We explain this in more detail later. We have also experimentally justified our choice by implementing classical work-stealing and comparing its performance over a randomly selected set of benchmarks with the double-ended queue based implementation. The experiments show that, in 40\% cases, classical work-stealing timed out whereas the double-ended queue based work stealing terminated. Furthermore, the instances where both terminated, the double-ended queue based work stealing was ~8.5 times faster.}

The server also maintains a queue of waiting clients, ones it could not reply to
immediately.

On receiving a message $\langle\texttt{SEND\_PARTITION}, \rho\rangle$, the
server stores the partition $\rho$ by pushing left into $Q[id]$. Because the
search on a client progressively inlines more procedures and makes more splits,
partitions towards the right of $Q[i]$ are the \textit{smallest}. Smallest
partitions incur least time to set up on a client (after it resets its solver).

On receiving a message
$\langle\texttt{GET\_PARTITION}\rangle$, the server enqueues the requesting
client in its waiting queue $wt$. The corresponding client waits
in an idle state until it receives a new partition from the server. Waiting
clients are served by the code shown in \linesref{l11}{l14}. It picks the
longest queue $Q[i]$, pops-right from it (to get the smallest partition in the
queue) and replies to a waiting client.

On receiving a message $\langle\texttt{POP}, id\rangle$, the server replies back
with either $\texttt{YES}$ or $\texttt{NO}$ depending on whether client $id$ can
be allowed to pop a partition from its local stack or not. Note that
partitions coming from client $i$ are pushed-left to $Q[i]$ and work is
delegated by popping-right. Thus, the last partition sent by $i$ must be the
left-most element of $Q[i]$. So if $Q[i]$ is non-empty, its left-most element is
removed and the client is told to proceed (\texttt{YES}).

Other than these messages, the server also listens to \texttt{OUTCOME} messages:
if any client reports \textsc{Unsafe} then all clients are terminated and the
\texttt{UnSafe} verdict is return to the user. The server returns \textsc{Safe}
verdict to the user when all queues in $Q$ are empty and all clients are idle
(i.e., $wt$ consists of all clients).


%\input{sections/splitrate}
%\begin{algorithm}
%\DontPrintSemicolon
%\KwIn{A Program $P$, $StepSize$}
%\KwOut{\textsc{Safe}, or \textsc{UnSafe}($\tau$)}
%id $\gets$ 0\;
%Q[0], $\dots$, Q[numClients] $\gets \emptyset, \dots, \emptyset$\;
%wt $\gets \emptyset$\;
%Q[0] $\gets P$
%%$startListening()$\\
%\While {true} {
%    r $\gets$ ReceiveMessage()\\
%    \If {r.query == $\langle$ \texttt{ID} $\rangle$} {
%        id $\gets$ id + 1\;
%        r.reply(id)\;
%        }
%    \ElseIf {r.query == $\langle\texttt{SEND\_PARTITION}, id, p\rangle$} {
%            $Q[id].PushLeft(p)$\;
%            \If {wt.count == 0} {
%                speed $\gets$ \texttt{LARGENUMBER}\;
%            }
%            \Else {
%                speed $\gets$ (Q[id].count/wt.count)*StepSize\;
%            }
%            r.reply(speed)\;
%        }
%    \ElseIf { r.query == $\langle\texttt{POP}, id \rangle$} {
%            \If {Q[id] $\neq \emptyset$} {
%                $r.reply(\texttt{YES})$\;
%                $Q[id].PopLeft();$\;
%            }
%            \Else {
%                $r.reply(\texttt{NO})$\\
%            }
%        }
%    \ElseIf {r.query == $\langle$ \texttt{GET\_PARTITION} $\rangle$} {
%            wt.enqueue(r)\;
%        }
%    \ElseIf {r.query == $\langle$ \texttt{OUTCOME}, outcome $\rangle$} {
%            \If {outcome == \textsc{UnSafe}} {
%                Ask Listener To Kill All Clients\;\todo{is there a single listener?}
%                \Return \textsc{UnSafe}($\tau$)\;
%            }
%            \Else {
%                r.reply(\texttt{CONTINUE})
%            }
%        }
%    \While {wt $\neq \emptyset \land {any}_i(Q[i].count > 0)$} {
%                i $\gets$ argmax Q[i].count\;
%                r $\gets$ wt.dequeue()\;
%                r.reply(Q[i].popRight())\;
%            }
%    \If {wt.count == numClients} {
%            Ask Listener To Kill All Clients\;
%                \Return \textsc{Safe}\;
%        }
%    \If {Exceeded(TimeBudget)} {
%        Ask Listener To Kill All Clients\;
%                \Return \textsc{Timedout}\;
%        }
%    }
%    \caption{Algorithm for server\todo{separete messages for listener and clients}}
%\label{server}
%\end{algorithm}



==> sections/methodology.tex <==
\section{Distributed Verification with $\toolname$}
\label{Se:Algorithm}

$\toolname$ parallelizes the stratified inlining algorithm so that it can be 
executed on multiple machines, making use of parallel compute and memory 
resources. $\toolname$ has multiple client processes and a single server process. All verification
happens on the client side. The server is a lightweight process that is merely responsible for coordination between the
clients. Each of the clients get a copy of the (same) program. The server asks one of the clients to
start the verification task. As the client proceeds, it can decide to split the search, creating two
sub-tasks (called \textit{partitions} in the discussion to follow). The client continues 
verifying one of the partitions and passes the other one to the server. The server receives and
stores the partitions that it gets from the clients in its internal datastructure. It then passes on the partitions to
available clients to parallelize the search.
Client processes do not coordinate with each other directly.

The paralellization introduces its own overhead and we must take care of reducing it as much as
possible. For instance, as clients finish one partition and start a new one, they incur a cost in
setting up search on the new partition. This setup time can be drastically reduced if a client 
picks up one of the partitions that it had produced itself. In this case, it simply relies on the
solver's incremental solving (via Push-Pop). Our client and server implementation makes use of this
optimization. 

We start by describing the client-side algorithm (\sectref{Client}) followed by the server-side
implementation (\sectref{Server}). These algorithms assume an arbitrary splitting heuristic (the
exact choice is immaterial for correctness of the algorithm). The heuristic that we used in
our implementation is explained in two parts: deciding when to split
(\sectref{SplitRate}) and what to split on (\sectref{SplittingHeuristic}).

\input{sections/client}

\paragraph{Must-reach constraint}
We now describe the construction of the must reach constraint, starting with the
single-procedure case. For a procedure
$p$, we use \textit{must-reach control variables} $r_l$, one for each block $l$.
Intuitively, setting $r_l$ to \textit{true} should mean that control must go
through block $l$. Recall from \sectref{Background} that the VC of a procedure uses
$i_l$ as a unique integer constant for block $l$ and $f$ as the control-flow
function. We define $\mr(p)$ as the following constraint:

\begin{equation} \label{Eqn:MustReach}
  \bigwedge_{l \in \blocks(p)} (r_l \Rightarrow \bigvee_{n \bpred(l)} (r_n
  \wedge f(i_l) == i_n))
\end{equation}

This constraint enforces that if a block $l$ must be reached, then one of its
predecessors must be reached. The use of the control-flow function ties this
constraint with the procedure's VC. 
For any block $l$, asserting $r_l \wedge \mr(p)$, in addition to the VC of $p$
will enforce the constraint that control \textit{must} pass through block $l$.
The proof is straightforward and we omit it from this paper.

To be more precise, we write $\mr(p, c)$ for the constraint $\mr(p)$ where the 
block identifiers $\{i_l\}$ are the same as the ones used in $\pVC(p, c)$.

For a dynamic callsite $c$, we construct $\mr(c)$ inductively over the length of
$c$. If $c = [\texttt{main}]$, then $\mr(c)$ is \textit{true}. Otherwise, if $c
= (l,p) :: c'$, then $\mr(c)$ is $r_l \wedge \mr(p, c') \wedge \mr(c')$. 



%We assume that the solver has support for computing \textit{unsatisfiability
%cores}; for $\Phi=\cup_{l \in L}\{\phi_i\}$, the solver returns the
%unsatisfiable core as the set of labels $\{l_i\}\subseteq L$ corresponding to
%all all the conjuncts $\phi_{l_i}$ such that $\Phi$ unsastisfiable.

\Omit{

\begin{algorithm}[ht]
%\SetAlgoLined
\DontPrintSemicolon
\KwIn{A callsite $C$ and a block $b \in C$}
\KwOut{Assert must-reach on $b$}
%Assert $C_0 \gets True$ \\
%Assert $C_b \gets True$ \\
$G \gets reverseDAG(procedureName(C))$\\
$N \gets TopologicalSort(G)$\\
bool $expr$;\\
\For{each node $n \in N$} {
    $expr \gets expr \land (\lor_{p \in Pred(n)} C_p)$
}
Assert($C_0 \land C_b \land expr$)
\caption{Assert mustreach}\label{mr}
\end{algorithm}
}

\input{sections/implementation}
\input{sections/heuristic} 
\input{sections/splitrate}


==> sections/splitrate.tex <==
\subsection{Adaptive Split Rate}
\label{Se:SplitRate}

This section describes the implementation of \lineref{whensplit} of
\algoref{Verify}: when to split the search.
Splitting is essential to obtain parallelism, however, splitting too much can
introduce unnecessary overheads. Ideally, we should split just enough to keep all
clients busy all the time. We control the rate of splitting in 
proportion to the number of idle clients, and inversely
proportional to the number of partitions already available at the server. In
other words, a client will split at a faster rate if there are a large number of idle
clients and the server has comparatively lesser number of partitions available.

Each client maintains a \textit{split time interval} $\delta$ (in seconds). 
It splits the search if $\delta$ seconds have elapsed since the last split.
The value of $\delta$ is initially $\delta_c$ (a fixed constant) but it can be updated
by the server. The server sends this value back as a reply to the
$\texttt{SEND\_PARTITION}$ message.
The server computes $\delta_i$ for a client $i$ as follows:

\begin{equation}\label{sprate}
\delta_i =
    \begin{cases}
      \frac{Q[i].count}{wt.count}\times \delta_c & \mbox{if } wt.count \neq 0 \\
      K \times \delta_c, & \mbox{otherwise}.
    \end{cases}
\end{equation}

In the first case, a client's splitting is slowed down in proportion to its queue size
(divided by the number of idle clients).
The second case applies when there are no idle clients. Increasing $\delta$ by a
factor of $K$ reduces the rate of splitting drastically. We use the values
$\delta_c=0.5s$ and $K=20$ in our experiments.

